Single-Branch Network Architectures to Close the Modality Gap in Multimodal Recommendation

Traditional recommender systems rely on collaborative filtering, using past user-item interactions to help users discover new items in a vast collection. In cold start, i.e., when interaction histories of users or items are not available, content-based recommender systems use side information instead. Hybrid recommender systems (HRSs) often employ multimodal learning to combine collaborative and side information, which we jointly refer to as modalities. Though HRSs can provide recommendations when some modalities are missing, their quality degrades. In this work, we utilize single-branch neural networks equipped with weight sharing, modality sampling, and contrastive loss to provide accurate recommendations even in missing modality scenarios by narrowing the modality gap. We compare these networks with multi-branch alternatives and conduct extensive experiments on three datasets. Six accuracy-based and four beyond-accuracy-based metrics help assess the recommendation quality for the different training paradigms and their hyperparameters in warm-start and missing modality scenarios. We quantitatively and qualitatively study the effects of these different aspects on bridging the modality gap. Our results show that single-branch networks achieve competitive performance in warm-start scenarios and are significantly better in missing modality settings. Moreover, our approach leads to closer proximity of an item's modalities in the embedding space. Our full experimental setup is available at https://github.com/hcai-mms/single-branch-networks.

==> resources/algorithms/item-sibrar.tex <==
\makeatletter
\newdimen\commentwd
\let\oldtcp\tcp
\def\tcp*[#1]#2{% only support one style for simplicity
    \setbox0\hbox{#2}%
    \ifdim\wd\z@>\commentwd\global\commentwd\wd\z@\fi
    \oldtcp*[r]{\leavevmode\hbox to \commentwd{\box0\hfill}}
}


\def\mytcp*[#1]#2{% only support one style for simplicity
    \setbox0\hbox{#2}%
    \ifdim\wd\z@>\commentwd\global\commentwd\wd\z@\oldtcp*[r]{\leavevmode\hbox to \commentwd{\box0\hfill}}\fi
    \ifdim\wd\z@<\commentwd\oldtcp*[r]{\leavevmode\hbox to \wd\z@{\box0\hfill}}\fi
}

\let\oldalgorithm\algorithm
\def\algorithm{\oldalgorithm
\global\commentwd\z@
\expandafter\ifx\csname commentwd@\romannumeral\csname c@\algocf@float\endcsname\endcsname\relax\else
\global\commentwd\csname commentwd@\romannumeral\csname c@\algocf@float\endcsname\endcsname
\fi
}
\let\oldendalgorithm\endalgorithm
\def\endalgorithm{\oldendalgorithm
\immediate\write\@auxout{\gdef\expandafter\string\csname commentwd@\romannumeral\csname c@\algocf@float\endcsname\endcsname{%
\the\commentwd}}}
    
    %\centering
    \begin{algorithm*}
        \DontPrintSemicolon
        \caption{Pseudocode for computing the batch loss in \sibrarItem}\label{alg:sibrar:train}
            \SetKwInOut{Input}{Input}            \SetKwInOut{Output}{Output}
            \SetKwFunction{negSampling}{negSampling}
            \SetKwFunction{randomSampling}{randomSampling}
            \Input{
                %$B = \{b | b \subset \{(u_i, i_j) | P_{ij}=1\}\}$: Batches of user--item training interactions\\
                $b \subset \{(u_i, i_j) | R_{ij}=1\}$: Batch of user--item training interactions\\
                $n_\text{neg}$: Number of negatives per interaction\\
                $\mathcal{M}^\text{item}$: Item training modalities\\
                \texttt{ctrEmbs}: Whether to use contrastive loss or not\\
                $\lambda, \tau$: Weight and temperature of contrastive loss
            }
            \Output{$\mathcal{L}$: Loss for the batch
            \vspace{-.9pt}}
%\scalebox{0.9}{
                $\mathcal{L}_\text{BPR} \leftarrow 0$ \tcp*[l]{Reset BPR Loss}
                $\mathcal{L}_\text{SInfoNCE} \leftarrow 0$ \tcp*[l]{Reset contrastive loss}
                \uIf{\texttt{ctrEmbs}}{$n_\text{mod} \leftarrow 2$}
                \Else{$n_\text{mod} \leftarrow 1$}
                \For{$(u_i, i_j)\in b$}{
                    $\mathbf{e_{i}} \leftarrow h(u_i)$\tcp*[l]{Embed user $u_i$}
                    $\mathcal{N}_{ij}\leftarrow$ \negSampling{$u_i, i_j, R$}\tcp*[l]{Sample negatives}
                    $\mathcal{M}_{ij}\leftarrow$ \randomSampling{$\mathcal{M}^{\text{item}}$}\tcp*[l]{Sample $n_\text{mod}$ training modalities}
                    %\For{$m \in \mathcal{M}_{ij}$}{
                    $\mathbf{e_{j}} \leftarrow \frac{1}{n_\text{mod}}\sum_{m\in \mathcal{M}_{ij}}g(m_j)$\tcp*[l]{Embed positive item $i_j$ with single-branch $g$ on modalities $\mathcal{M}_{ij}$}
                    $\hat{y}_{ij} \leftarrow \mathbf{e_{i}}\cdot\mathbf{e_{j}}$\tcp*[l]{Compute positive logit}
                    \For{$i_k \in \mathcal{N}_{ij}$}{
                        $\mathbf{e_{k}} \leftarrow \frac{1}{n_\text{mod}}\sum_{m\in \mathcal{M}_{ij}}g(m_k)$\tcp*[l]{Embed item $i_k$ with single-branch $g$ on modalities $\mathcal{M}_{ij}$}
                        $\hat{y}_{ik} \leftarrow \mathbf{e_{i}}\cdot\mathbf{e_{k}}$\tcp*[l]{Compute negative logit}
                        $\mathcal{L}_\text{BPR} \leftarrow \mathcal{L}_\text{BPR} + \ln{\sigma(\hat{y}_{ij} - \hat{y}_{ik})}$ \tcp*[l]{Accrete BPR loss}
                    }
                    \If{\texttt{ctrEmbs}}{
                                $\mathcal{L}_\text{SInfoNCE} \leftarrow \mathcal{L}_\text{SInfoNCE} - \ln{\frac{\mathrm{e}^{(g(m^{j}_1) \cdot g(m^{j}_2))/\tau}}{\sum_{k \in \{j\}\cup \mathcal{N}_{ij}}\mathrm{e}^{(g(m^{j}_1) \cdot g(m^{k}_2))/\tau}}} - \ln{\frac{\mathrm{e}^{(g(m^{j}_2) \cdot g(m^{j}_1))/\tau}}{\sum_{k \in \{j\}\cup \mathcal{N}_{ij}}\mathrm{e}^{(g(m^{j}_2) \cdot g(m^{k}_1))/\tau}}}$\mytcp*[l]{Accrete contrastive loss}
                    }
                    $\mathcal{L} \leftarrow \mathcal{L}_\text{BPR} + \lambda \mathcal{L}_\text{SInfoNCE}$
                }
            %}
    \end{algorithm*}
